MatCLIP: Light- and Shape-Insensitive Assignment of PBR Material Models

Assigning realistic materials to 3D models remains a significant challenge in computer graphics. We propose MatCLIP, a novel method that extracts shape- and lighting-insensitive descriptors of Physically Based Rendering (PBR) materials to assign plausible textures to 3D objects based on images, such as the output of Latent Diffusion Models (LDMs) or photographs. Matching PBR materials to static images is challenging because the PBR representation captures the dynamic appearance of materials under varying viewing angles, shapes, and lighting conditions. By extending an Alpha-CLIP-based model on material renderings across diverse shapes and lighting, and encoding multiple viewing conditions for PBR materials, our approach generates descriptors that bridge the domains of PBR representations with photographs or renderings, including LDM outputs. This enables consistent material assignments without requiring explicit knowledge of material relationships between different parts of an object. MatCLIP achieves a top-1 classification accuracy of 76.6%, outperforming state-of-the-art methods such as PhotoShape and MatAtlas by over 15 percentage points on publicly available datasets. Our method can be used to construct material assignments for 3D shape datasets such as ShapeNet, 3DCoMPaT++, and Objaverse. All code and data will be released.

==> figs/ablation/ablation.tex <==
\begin{figure}[t]
    \centering
     \includegraphics[width=\linewidth,trim={0.8cm 0.25cm 1.25cm 1.45cm},clip]{figs/ablation/ablation_v1.pdf}
    \caption{Ablation study examining the effect of shape and environment map diversity on classification accuracy. The full model, which uses all six shapes and seven environment maps (42 renderings per material), performs best. Variants include: 'Plane 1 Env,' using a single shape (plane) and one environment map; 'Plane 7 Env,' using the plane with all seven environment maps; and 'All Shapes 1 Env,' using all six shapes with a single environment map.}
    \label{fig:ablation}
\end{figure}

==> figs/results_chatgpt/results_chatgpt.tex <==
\newcommand{\secondnodedist}{25mm}

\begin{figure}[t]
    \centering
\begin{tikzpicture}[node distance=0.5cm, every node/.style={font=\sffamily}]

    % Image node
    \node[anchor=north west] (image) at (0,0) {\includegraphics[width=0.125\textwidth]{figs/results_flux_variations/flux/0c_42b_00007.png}};

        % User messages (right of image, aligned with msg2)
    \node[draw=none, fill=gray!20, rounded corners, align=left, text width=55mm, anchor=north west, right=0.05cm of image] (msg1) { \small
This image was generated by an LDM using the prompt "A photograph of a very comfortable chair, high quality, white background." Please suggest 3 different prompts to obtain more meaningful but very differently looking results that take the geometry into account.};

    % ChatGPT messages (below image and msg1)
    \node[draw=none, fill=gray!40, rounded corners, align=left, text width=80mm, anchor=north west] (msg2) at (0,-\secondnodedist) { \small
Here are three alternative prompts you can use to generate varied but geometrically related chairs using a latent diffusion model:
        \begin{enumerate}
            \item \emph{A futuristic armchair inspired by mid-century modern design, featuring metallic legs and a sleek seat.}
            \item \emph{A luxurious lounge chair with an organic design, curved lines, and upholstered with soft velvet fabric.}
            \item \emph{A modern Scandinavian-style chair with a minimalist wooden frame, light fabric cushions, and angled legs.}
        \end{enumerate}
    };
% (0,-25mm)

\end{tikzpicture}
    \caption{We exploit ChatGPT to obtain various prompts we then use to condition Flux. Top to bottom: The query target image, our query prompt, and the response from ChatGPT representing a set of advanced prompts we use to obtain the material variations shown in Fig.~\ref{fig:results_flux_variations}, middle row.}
    \label{fig:chatgpt}
\end{figure}


==> figs/results_flux_variations/results_chatgpt_flux_variations_merged.tex <==
\renewcommand{\imgwidth}{0.132}
\renewcommand{\imgskip}{0.5mm}
\newcommand{\vlabel}[1]{\raisebox{11mm}{\rotatebox[origin=c]{90}{#1}}}
\newcommand{\secondnodedist}{9mm}

\begin{figure*}[btp]
  \centering
  \begin{tabular}{@{}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{}}
    % Row 1: Label, image, empty, TikZ chat block spanning 5 columns
    \multicolumn{9}{c}{
      \begin{tikzpicture}[node distance=0.5cm, every node/.style={font=\sffamily}]
        % User message
        \node[draw=none, fill=gray!20, rounded corners, align=left, text width=170mm, anchor=north west] (msg1) at (0,0) { \small
This image was generated by an LDM using the prompt "A photograph of a very comfortable chair, high quality, white background." Please suggest 3 different prompts to obtain more meaningful but very differently looking results that take the geometry into account.};

        % ChatGPT response
        \node[draw=none, fill=gray!40, rounded corners, align=left, text width=170mm, anchor=north west] (msg2) at (0,-\secondnodedist) { \small
Here are three alternative prompts you can use to generate varied but geometrically related chairs using a latent diffusion model:
            \begin{enumerate}
                \item \emph{A futuristic armchair inspired by mid-century modern design, featuring metallic legs and a sleek seat.}
                \item \emph{A luxurious lounge chair with an organic design, curved lines, and upholstered with soft velvet fabric.}
                \item \emph{A modern Scandinavian-style chair with a minimalist wooden frame, light fabric cushions, and angled legs.}
            \end{enumerate}
        };
      \end{tikzpicture}
    } \\

    \vlabel{Target Shape} & \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/flux/0c_42b_00007.png} &
    % Row 2: Regular Prompt
    \vlabel{Regular Prompt} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00026.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00031.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00046.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00022.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00049.png} & \\

    % Row 3: Advanced Prompt
    & & \vlabel{Advanced Prompt} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_007_00000.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_000_00001.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_018_00000.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_019_00000.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_015_00003.png} & \\

    % Row 4: Outliers
    & & \vlabel{Outliers} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_015_00001.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_031_00001.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_034_00003.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_075_00002.png} &
    \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_099_00000.png} &
  \end{tabular}

  \caption{We use ChatGPT to expand the prompt space for Flux \cite{flux2023}. Row 1 shows the target shape and the prompt engineering dialog. Rows 2–4 show results generated using regular prompts (top), advanced prompts (middle), and outlier cases (bottom). Advanced prompts enhance design diversity but may introduce unintended artifacts.}
  \label{fig:final_merged_flux_chat}
\end{figure*}


==> figs/results_flux_variations/results_flux_variations.tex <==
\renewcommand{\imgwidth}{0.132}
\renewcommand{\imgskip}{0.5mm}
\renewcommand{\tupleskip}{4mm}

\renewcommand{\imageflux}[1]{\includegraphics[width=\imgwidth\textwidth, trim={0 0 538px 0}, clip]{#1}}
\renewcommand{\imageours}[1]{\includegraphics[width=\imgwidth\textwidth, trim={538px 0 0 0}, clip]{#1}}

% \newcommand{\vlabel}[1]{\raisebox{0.5\height}{\rotatebox[origin=c]{90}{\strut #1}}}
% \newcommand{\vlabel}[1]{\raisebox{0.5\height}{#1}}

%\newcommand{\vlabel}[1]{#1}

\newcommand{\vlabel}[1]{\raisebox{11mm}{\rotatebox[origin=c]{90}{#1}}}

% Define a new column type 'm' for vertical centering with fixed height
% \newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

\begin{figure*}[btp]
  \centering
    \begin{tabular}{@{}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{\hskip \imgskip}c@{}} 
        % FLUX & Ours & FLUX & Ours & FLUX & Ours & FLUX & Ours \\
        \vlabel{Target Shape} &
        % \rotatebox[origin=l]{90}{Target Shape} & 
        % \rotatebox[origin=c]{90}{\raisebox{0.5\height}{Target Shape}} &
        % \rotatebox[origin=l]{90}{Target Shape} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/flux/0c_42b_00007.png} &
        \vlabel{Regular Prompt} &
        % \rotatebox[origin=l]{90}{Regular Prompt} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00026.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00031.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00046.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00022.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_regular/0c_42b_00049.png} \\
        & & \vlabel{Advanced Prompt} &
        % & &\rotatebox[origin=l]{90}{Advanced Prompt} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_007_00000.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_000_00001.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_018_00000.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_019_00000.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced/0c_42b_015_00003.png} \\
        & & \vlabel{Outliers} &
        % & &\rotatebox[origin=l]{90}{Outliers} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_015_00001.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_031_00001.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_034_00003.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_075_00002.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours_advanced_outliers/0c_42b_099_00000.png} 
        
        % \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours/0c_42b_011_00000.png} &
        % [\tupleskip]
        % \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours/0c_42b_015_00000.png} &

        % \includegraphics[width=\imgwidth\textwidth]{figs/results_flux_variations/ours/0c_42b_018_00000.png} &
    \end{tabular}
    \caption{Exploring a larger material design space for one particular shape using Flux~\cite{flux2023} and ChatGPT-suggested prompts as described in Section \ref{sec:chatgpt}. While regular prompts mostly lead to basic designs (top row), we use the obtained advanced prompts to obtain more variability (middle row). While advanced prompts extend the design space, they occasionally produce unusual designs (bottom row).}
    \label{fig:results_flux_variations}
\end{figure*}

%  and 
% \ref{fig:chatgpt}.

%  and Fig.~\ref{fig:chatgpt}
% # 1 of the supplementary materials

==> figs/results_ours/results_ours_old.tex <==
\newcommand{\imgwidth}{0.2755}

\begin{figure*}
  \centering
  \setlength{\tabcolsep}{1em} % Adjust spacing between images
    \renewcommand{\arraystretch}{1.5} % Adjust row spacing
    \begin{tabular}{ccc}
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_00d_00006.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_015_00048.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_024_00027.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_088_00024.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_0ad_00052.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_0b8_00036.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_0c4_00040.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_0db_00025.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_438_00042.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_0f8_00028.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_0fd_00047.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_15d_00019.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_16a_00000.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_176_00040.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_178_00010.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_1a7_00056.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_1b3_00002.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_1b4_00026.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_1d0_00020.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_1ed_00011.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_1fe_00061.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_432_00026.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_20b_00024.png} & 
        \includegraphics[width=\imgwidth\textwidth]{figs/results_ours/0c_2ac_00025.png} \\
    \end{tabular}
    \caption{Matching materials from Stable Diffusion output images to materials of our material database using our MatCLIP model. Each pair shows the output from Stable Diffusion (left side) and a rendering of the same shape with the materials matched by our MatCLIP (right side).}
    \label{fig:results_ours}
\end{figure*}



==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> table_eval.tex <==
\begin{table*}[t]
\begin{tabular}{l|c|c|}
                                                                          & \multicolumn{2}{c}{\textbf{Validation Accuracy [\%] $\uparrow$}}                                          \\
                                                                          & \multicolumn{1}{c}{\textbf{Top-1}} & \multicolumn{1}{c}{\textbf{Top-5}}                                   \\
% \textbf{Closed Set (1598 MatSynth Materials)}     & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}        &  &  \\
\hline
PhotoShape (ResNet-34)                                                    & 57.21                                               & 77.39                                               \\
PhotoShape (ResNet-50)                                                    & 58.76                                               & 77.62                                               \\
PhotoShape (ViT-B/16)                                                     & 60.86                                               & 78.23                                               \\
\hline
OpenCLIP (Max. Inscribed Square Crop, Max. Score to 42 Material Features) & 16.13                                               & 31.49                                               \\
OpenCLIP (Max. Inscribed Square Crop, Avg. Material Features)             & 19.90                                               & 35.34                                               \\
\hline
% MatAtlas (0.5 * LAB + 0.5 * CLIP) (Max. Score to 42 Material Features)    & 18.30                                               & 34.71                                               \\
MatAtlas (0.8 * LAB + 0.2 * CLIP) (Max. Score to 42 Material Features)    & 18.77                                               & 36.79                                               \\
% MatAtlas (0.5 * LAB + 0.5 * CLIP) (Average Material Features)             & 20.35                                               & 37.70                                               \\
MatAtlas (0.8 * LAB + 0.2 * CLIP) (Average Material Features)             & 13.14                                               & 28.40                                               \\
\hline
\textbf{MatCLIP (Ours)}                                                    & \textbf{76.69}                                      & \textbf{89.02}
\end{tabular}
\caption{Quantitative evaluation of our method. We compare to variants of PhotoShape \cite{photoshape2018}, simple crop matching using CLIP \cite{radford2021_clip}, and variants of the core method of MatAtlas \cite{matatlas2024}.}.
\label{tab:table_eval}
\end{table*}

==> table_eval_v2.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{Top-1 Accuracy [\%] $\uparrow$} & \textbf{Top-5 Accuracy [\%] $\uparrow$} \\
\midrule
PhotoShape (ResNet-34) & 57.21 & 77.39 \\
PhotoShape (ResNet-50) & 58.76 & 77.62 \\
PhotoShape (ViT-B/16) & 60.86 & 78.23 \\
\midrule
OpenCLIP (Max. Inscribed Square Crop, Max. Score to 42 Material Features) & 16.13 & 31.49 \\
OpenCLIP (Max. Inscribed Square Crop, Avg. Material Features) & 19.90 & 35.34 \\
\midrule
MatAtlas (0.8 × LAB + 0.2 × CLIP, Max. Score to 42 Material Features) & 18.77 & 36.79 \\
MatAtlas (0.8 × LAB + 0.2 × CLIP, Avg. Material Features) & 13.14 & 28.40 \\
\midrule
\textbf{MatCLIP (Ours)} & \textbf{76.69} & \textbf{89.02} \\
\bottomrule
\end{tabular}
\caption{
Quantitative evaluation of our method. We compare to variants of PhotoShape \cite{photoshape2018}, simple crop matching using CLIP \cite{radford2021_clip}, and variants of the core method of MatAtlas \cite{matatlas2024}. We either average or identify the max. score across the 42 material features of each of our materials in case of CLIP and MatAtlas. Accuracy is evaluated on Top-1 and Top-5 metrics, with higher values indicating better performance.
}
\label{tab:table_eval}
\end{table*}

==> table_manual_annotation.tex <==
\begin{table}[]
\begin{tabular}{l|r|r|}
                            & \textbf{Val.Acc. {[}\%{]} $\uparrow$} \\
\hline

PhotoShape (ResNet-34)      & 46.67 \\ % & xx.xx \\
PhotoShape (ResNet-50)      & 49.07 \\ % & xx.xx \\
PhotoShape (ViT-B/16)       & 44.27 \\ % & xx.xx \\
\hline
OpenCLIP (Max. Score)       & 49.20 \\ % & 48.93 \\
OpenCLIP (Avg. Features)    & 44.65 \\ % & 38.50 \\
\hline
% MatAtlas (0.5 / 0.5) (Max.) & 53.21 \\ % & 44.65 \\
MatAtlas (0.8 / 0.2) (Max.) & 52.94 \\ % & 44.39 \\
% MatAtlas (0.5 / 0.5) (Avg.) & 58.29 \\ % & 45.45 \\
MatAtlas (0.8 / 0.2) (Avg.) & 48.93 \\ % & 39.84 \\
\hline
MatCLIP (Ours)      & \textbf{55.47} % & \textbf{xx.xx}
\end{tabular}
\caption{Model comparison using manually annotated ground-truth data. We evaluate the performance to assign the correct substance derived from matched materials. % Top-5 is considered right only if at least 3 of the best-matched materials belong to the ground truth substance.
We use the same models as in Table \ref{tab:table_eval}.}
\label{tab:manual_annotation}
\end{table}

==> table_manual_annotation_v2.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lc}
\toprule
\textbf{Method} & \textbf{Val.Acc. [\%] $\uparrow$} \\
\midrule
PhotoShape (ResNet-34) & 46.67 \\
PhotoShape (ResNet-50) & 49.07 \\
PhotoShape (ViT-B/16) & 44.27 \\
\midrule
OpenCLIP (Max. Score) & 49.20 \\
OpenCLIP (Avg. Features) & 44.65 \\
\midrule
MatAtlas (0.8 × LAB + 0.2 × CLIP, Max.) & 52.94 \\
MatAtlas (0.8 × LAB + 0.2 × CLIP, Avg.) & 48.93 \\
\midrule
\textbf{MatCLIP (Ours)} & \textbf{55.47} \\
\bottomrule
\end{tabular}
\caption{
Model comparison using manually annotated ground-truth data. We evaluate the performance of assigning the correct substance derived from matched materials. We use the same models as in Table~\ref{tab:table_eval}.
}
\label{tab:manual_annotation}
\end{table}

